Graph Size Estimation

Many online networks are not fully known and are often studied via sampling. Random Walk (RW) based techniques are the current state-of-the-art for estimating nodal attributes and local graph properties, but estimating global properties remains a challenge. In this paper, we are interested in a fundamental property of this type - the graph size N, i.e., the number of its nodes. Existing methods for estimating N are (i) inefficient and (ii) cannot be easily used with RW sampling due to dependence between successive samples. In this paper, we address both problems. First, we propose IE (Induced Edges), an efficient technique for estimating N from an independence sample of graph's nodes. IE exploits the edges induced on the sampled nodes. Second, we introduce SafetyMargin, a method that corrects estimators for dependence in RW samples. Finally, we combine these two stand-alone techniques to obtain a RW-based graph size estimator. We evaluate our approach in simulations on a wide range of real-life topologies, and on several samples of Facebook. IE with SafetyMargin typically requires at least 10 times fewer samples than the state-of-the-art techniques (over 100 times in the case of Facebook) for the same estimation error.

==> star_sampling.tex <==







\section{Appendix: Star sampling}\label{sec:Star sampling}

\maciej{Works not so well, so temporarily in the Appendix}

\maciej{What about using node sampling without replacements? Might work great!}

\subsection{UIS}
If $S$ is chosen independently, uniformly at random (with repetitions) from $V$ (\ie $S$ is a UNI sample), then the nodes in $\mathcal{N}(S)$ are subject to linear bias towards higher node degrees (\ie exactly the same as RW). 
In other words, every node $v\in\mathcal{N}(S)$ is sampled with probability proportional to its degree~$k_v$.

In that case, we can try to interpret $\mathcal{N}(S)$ as our sample $S$ and plug it in the estimator~\eqn{eq:est_N WWW}. So we have $S \leftarrow\mathcal{N}(S)$

We can use \eqn{eq: n^col} to count the number of collisions~$n^\col$. 
\maciej{A slightly better formula (especially for small $S$) should take into account that, by construction, collisions between nodes in $\mathcal{N}(v)$ are not possible, which reduces the number of collisions observed in $\mathcal{N}(S)$. TODO}

In contrast, we cannot directly use 
$\Psi_{1} = \sum_{v\in \mathcal{N}(S)} \deg(v)$, 
because we know $\deg(v)$ only for nodes $v\in S$. However, we can write
$$\Psi_{1} = |\mathcal{N}(S)| \cdot \Angles{q_k}, $$
where $\Angles{q_k}$ is the average node degree in $\mathcal{N}(S)$. 
Because nodes in $\mathcal{N}(S)$ are linearly biased towards higher degrees, we can estimate $\Angles{q_k}$ by 
\begin{equation}
	\Angles{q_k} = \sum_k k\, q_k = \frac{\sum_k k^2\, p_k}{\Angles{k}} = \frac{\Angles{k^2}}{\Angles{k}},
\end{equation}
where $\Angles{k^2}$ is the average squared node degree in (original UNI) $S$. 
So
\begin{eqnarray}
\label{eq:PSI 1 UNI}	\Psi_{1} &\cong & |\mathcal{N}(S)| \cdot \frac{\displaystyle\sum_{v\in S} \deg^2(v)}{\displaystyle\sum_{v\in S} \deg(v)},\\
\label{eq:PSI-1 UNI}	\Psi_{-1} &\cong & |\mathcal{N}(S)| \cdot \frac{\displaystyle|S|}{\displaystyle\sum_{v\in S} \deg(v)}.
\end{eqnarray}
%
\maciej{Btw, $|\mathcal{N}(S)| = \sum_{v\in S} k_v$.}
\maciej{Try to integrate the basic nodes too!}







 
 
 
\subsection{WIS}
Under WIS, we have to re-weight~$S$ to UNI, which lets us interpret~$\mathcal{N}(S)$ as RW sample and apply the formulas from the previous subsection. 

First, we re-weight \eqn{eq: n^col} to obtain a the number of collisions~$n^\col$ corrected for the WIS bias:
%\begin{equation}\label{eq: n^col WIS}
%	n^\col = {|\mathcal{N}(S)|\choose 2}\ 
%	\left(\sum_{i\neq j} \frac{1_{\{v_i=v_j\}}}{\w(v_i)\, \w(v_j)}\right)\ 
%	\left(\sum_{i\neq j} \frac{1}{\w(v_i)\, \w(v_j)}\right)^{-1}
%\end{equation}
\begin{equation}\label{eq: n^col WIS}
	n^\col \ =\  {|\mathcal{N}(S)|\choose 2}\ \cdot \ 
	\frac  {\displaystyle \sum_{i\neq j} \frac{1_{\{v_i=v_j\}}}{\w(v_i)\, \w(v_j)}}  {\displaystyle \sum_{i\neq j} \frac{1}{\w(v_i)\, \w(v_j)}}
\end{equation}
%
We obtain $\Psi_{1}$ and $\Psi_{-1}$ by re-weighting \eqn{eq:PSI 1 UNI} and \eqn{eq:PSI-1 UNI}, respectively:
\begin{eqnarray}
	\Psi_{1} &\cong & |\mathcal{N}(S)| \cdot \frac{\displaystyle \sum_{v\in S} \frac{\deg^2(v)}{\w(v)}}{\displaystyle\sum_{v\in S} \frac{\deg(v)}{\w(v)}},\\
	\Psi_{-1} &\cong & |\mathcal{N}(S)| \cdot \frac{\displaystyle\sum_{v\in S} \frac{1}{\w(v)}}{\displaystyle\sum_{v\in S} \frac{\deg(v)}{\w(v)}}.
\end{eqnarray}




%\displaystyle
